Unraveling Parameter Degeneracy in GRB Data Analysis

Gamma-ray burst (GRB) afterglow light curves and spectra provide information about the density of the environment, the energy of the explosion, the properties of the particle acceleration process, and the structure of the decelerating jet. Due to the large number of parameters involved, the model can present a certain degree of parameter degeneracy. In this paper, we generated synthetic photometric data points using a standard GRB afterglow model and fit them using the Markov Chain Monte Carlo (MCMC) method. This method has emerged as the preferred approach for analysing and interpreting data in astronomy. We show that, depending on the choice of priors, the parameter degeneracy can go unnoticed by the MCMC method. Furthermore, we apply the MCMC method to analyse the GRB~170817A afterglow. We find that there is a complete degeneracy between the energy of the explosion $E$, the density of the environment $n$, and the microphysical parameters describing the particle acceleration process (e.g. $\epsilon_e$ and $\epsilon_B$), which cannot be determined by the afterglow light curve alone. Our results emphasise the importance of gaining a deep understanding of the degeneracy properties which can be present in GRB afterglows models, as well as the limitations of the MCMC method. In the case of GRB 170817, we get the following values for the physical parameters: $E=8\times 10^{50}-1 \times 10^{53}$ erg, $n=7\times 10^{-5}-9\times10^{-3}$, $\epsilon_e=10^{-3}-0.3$, $\epsilon_B=10^{-10}-0.3$.

==> oldtext.tex <==
% GRB most used in papers, then it is most usual to see degeneration problems in this GRB.
% Check literature and see what happens with MCMC in other GRBs, if they are degenerated they will be added to the discussion (more generally) with the referee recomendation: "In the case of GRB 170817A the entire radio to X-ray afterglow spectrum lies on the same spectral segment, and this makes the degeneracy problem more severe. However, the degeneracy can be identified on other GRBs, such as <> (ref) or <> (ref)."

% Also we can add the papers reviewed in the WhatsApp group with misleading use of MCMC (i.e., Ryan paper with more then 15 fitted params and <search other>)

% Papers with degeneracy in MCMC:
% GRB230812B: Hussenot-Desenonges, T. https://ui.adsabs.harvard.edu/abs/2023arXiv231014310H/abstract
% GRB 170817A: Ryan https://ui.adsabs.harvard.edu/abs/2023arXiv231002328R/abstract
% GRB 221009A: Laskar https://ui.adsabs.harvard.edu/abs/2023ApJ...946L..23L/abstract
% GRB 210104A: Zhang https://ui.adsabs.harvard.edu/abs/2022ApJ...941...63Z/abstract
% GRB 210205A: Gupta https://ui.adsabs.harvard.edu/abs/2022JApA...43...11G/abstract
% Fraija: https://ui.adsabs.harvard.edu/abs/2020ApJ...896...25F/abstract
% GRB 160625B: Cunningham https://ui.adsabs.harvard.edu/abs/2020ApJ...904..166C/abstract




%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
% figura anterior
\begin{figure}
    \includegraphics[width=\linewidth]{Figures/cornerplot_GRB_order2_1.png}
      \includegraphics[width=.95\linewidth]{Figures/autocorrelation_GRB_order2_1.png}
  \caption{
\emph{Top panel:} Corner plot obtained in MCMC on the degenerated model function (equation \ref{eq:order2}) using {\sc emcee} \citep{Foreman2013}. Labels $k, \epsilon_\mathrm{e},~p$ correspond to the fitted coefficients in the model. The truth values of the synthetic data are shown with red lines.
\emph{Bottom panel:} Autocorrelation plot obtained for the MCMC routine of the model in equation \ref{eq:order2}. The black dashed line represents the threshold $N = 100n$, with $n$ the number of iterations of MCMC. The red line represents the average autocorrelation time $\tau$ estimated by {\sc emcee}. The dotted lines represent the autocorrelation time for the parameters $\alpha$ (blue line), $\epsilon_\mathrm{e}$ (green line) and $p$ (magenta line). }
     \label{fig:GRBfit2}
\end{figure}
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%


 %One of the advantages over traditional MCMC sampling methods is the invariance to linear transformations of the parameter space \citep{Foreman2013}.
%{\bf que significa esto y porque lo ponemos?} 
%This property implies that we could construct a solution with parameters that are a linear transformation of the original parameters (for example, in the context of the fireball model), and we would still obtain the same result. Therefore, the {\sc emcee} is insensitive to covariance between parameters and does not have performance disadvantages in implementations using a set of linear transformations of the parameters. %The performance of this code is specified by the autocorrelation time, a parameter that quantifies how many steps are needed for the sampler to \emph{forget} where it started.


\begin{itemize}
    %\item small intro to grb 170817a
    %\item \textcolor{purple}{discuss the fit by makhatini However, it can be mentioned that there are events that are observed by different instruments and facilities that obtain data in different ranges of the electromagnetic spectrum. Thus, the GRB 170817A can be studied and modelled in detail by \citet{Makhathini2021}, avoiding a degenerate problem by applying the MCMC technique to only find 6 parameters in its model.}

    %\item  \textcolor{purple}{show the fit and the associated degeneracy}
    %\item  \textcolor{purple}{conclude the section saying that fitting the GRB 170817A light curves using more than six parameters leads to misleading/wrong results. The determination of density, energy and microphysical parameters remains uncertain for this grb. Discuss how polarization can not help to resolve the degeneracy. Maybe VLBI observations can help, detailed modelling is needed. We leave it to future work}
\end{itemize}



% Hacer discusión acerca de como cambian los parámetros, por qué y el como influye el ruido sobre los resultados de los fittings (en la figura 1 los puntos del fit en los paneles izquierdo y derecho no son exactamente iguales, lo hice a propósito para añadir el análisis del ruido que se discutió en la sesión del 26 de Junio)

\begin{table*}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
       & $a$                     & $b$                     & $c$                     & $d$                     & $e$                     \\ \hline
truths & $-1$                    & $1$                     & $-0.5$                  & $2.5$                   & $-0.7$                  \\
run1   & $-1.69^{+0.29}_{-0.30}$ & $-5.33^{+1.33}_{-1.32}$ & $-6.48^{+1.77}_{-1.78}$ & $-5.73^{+0.90}_{-0.89}$ & $-1.29^{+0.15}_{-0.15}$ \\ 
run2   & $-1.11^{+0.32}_{-0.32}$ & $2.74^{+1.41}_{-1.44}$  & $-3.95^{+1.87}_{-1.86}$ & $4.83^{+0.91}_{-0.92}$  & $-1.18^{+0.15}_{-0.15}$ \\ \hline
\end{tabular}
\caption{Parameters estimated from the MCMC fitting of a 4th-order polynomial. The truth values are presented in the first row.}
\label{tab:table1}
\end{table*}

\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=\linewidth]{Figures/Quartic_fit_1.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=\linewidth]{Figures/Quartic_fit_2.png}
     \end{subfigure}
     \caption{Best fit results obtained for two runs of MCMC in a 4th-order function (left panel run1, right panel run2). We present the true synthetic model (red line), the model with added Gaussian noise and uncertainties (black points) and the best-fit function obtained from MCMC (blue line). The $1\sigma$ error of the fit is represented by the blue shaded area.}
     \label{fig:figure1}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{Figures/Quartic_fit_1_corner.png}
    \caption{Corner plots obtained from the MCMC in a 4th-order function using {\sc Emcee} \citep{Foreman2013} corresponding to the parameters listed in Table~\ref{tab:table1}. Top panel: run1, bottom panel: run2. The blue lines represent the truth values of the synthetic data.}
\end{figure*}
\begin{figure*}\ContinuedFloat
    \centering
    \includegraphics[width=\linewidth]{Figures/Quartic_fit_2_corner.png}
     \caption{(Continued) Cornerplots obtained for two runs of MCMC (left panel run1, right panel run2) in a 4th-order function using Emcee \citep{Foreman2013}. The labels $a,~b,~c,~d,~e$ correspond to the polynomial coefficients from 0th to 4th respectively. The blue lines represent the truth values of the synthetic data.}
     \label{fig:corner1}
\end{figure*}






\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.45\linewidth}
         \centering
         \includegraphics[width=\linewidth]{Figures/cornerplot_GRB_order2_1.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.54\linewidth}
         \centering
         \includegraphics[width=\linewidth]{Figures/autocorrelation_GRB_order2_1.png}
     \end{subfigure}
     \caption{\textbf{Left:} Cornerplot obtained in MCMC on the degenerated model function (equation \ref{eq:order2}) using Emcee \citep{Foreman2013}. Labels $k, \epsilon_\mathrm{e},~p$ correspond to the fitted coefficients in the model. The blue lines represent the truth values of the synthetic data. \textbf{Right:} Autocorrelation plot obtained for the MCMC routine of the model in equation \ref{eq:order2}. The black dashed line represents the threshold $N = 100n$, with $n$ the number of iterations of MCMC. The blue line represents the autocorrelation $\tau$ estimated by Emcee.}
    \label{fig:cornerGRB2}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.6\linewidth]{Figures/Fit_GRB_order2_1.png}
    \caption{Best fit results obtained using MCMC in the model function of equation \ref{eq:order2}. The true synthetic model is represented with ** line, and the black points represent the model with added Gaussian noise and uncertainties. The best fit function and the uncertainties $1\sigma$ obtained from MCMC are represented with the red line and shaded area.}
     \label{fig:GRBfit2}
\end{figure*}




\subsection{Fourth Degree Polynomial Model}
\label{sec:fourth}

We demonstrate the impact of fitting a degenerate model using MCMC, by considering a simple model of a fourth-degree polynomial function. As can be seen in Figure~\ref{fig:figure1}, we implement a model described by:
\begin{eqnarray}
    y(x) = -\frac{7}{10}x^4 + \frac{5}{2} x^3 - \frac{x^2}{2} + x - 1,
\end{eqnarray}

with added Gaussian noise and uncertainties. We try to fit a structure as follows:
\begin{eqnarray}
    y(x) = ex^4 + dx^3 + cx^2 + bx + a,
\end{eqnarray}

where $a,~b,~c,~d,~e$ are constant free parameters. We chose 100 walkers and flat priors on all the parameters. Furthermore, we monitor the progress of the chain using an autocorrelation time $\tau$ criterion\footnote{This parameter quantifies how many steps are needed for the sampler to “forget” where it started \citep{Foreman2013}} \citep{Foreman2013} that is updated every 100 steps. Therefore, we stop the sampler if the Markov chain has a length $L$ with $L\geq100\tau$ and if $\tau$ has not changed by more than $1\%$. In this way, the convergence of the Markov chain is ensured, removing the need to use a fixed number of steps. The initial guess for the walkers is initialised from a standard normal distribution with mean and variance values of $0$ and $1$, respectively.

We present the results of two executions of the same MCMC procedure: The first execution (hereafter run1) converged after $7700$ steps, and the second execution (hereafter run2) converged at $6900$ steps. The best-fit parameters for run1 and run2 are presented in Table~\ref{tab:table1}. We illustrate in Figure~\ref{fig:figure1} the best fit polynomials obtained, whereas in Figure~\ref{fig:corner1}, we present their corresponding corner plots.

